Rethinking Model Selection and Decoding for Keyphrase Generation with Pre-trained Sequence-to-Sequence Models

Keyphrase Generation (KPG) is a longstanding task in NLP with widespread applications. The advent of sequence-to-sequence (seq2seq) pre-trained language models (PLMs) has ushered in a transformative era for KPG, yielding promising performance improvements. However, many design decisions remain unexplored and are often made arbitrarily. This paper undertakes a systematic analysis of the influence of model selection and decoding strategies on PLM-based KPG. We begin by elucidating why seq2seq PLMs are apt for KPG, anchored by an attention-driven hypothesis. We then establish that conventional wisdom for selecting seq2seq PLMs lacks depth: (1) merely increasing model size or performing task-specific adaptation is not parameter-efficient; (2) although combining in-domain pre-training with task adaptation benefits KPG, it does partially hinder generalization. Regarding decoding, we demonstrate that while greedy search achieves strong F1 scores, it lags in recall compared with sampling-based methods. Based on these insights, we propose DeSel, a likelihood-based decode-select algorithm for seq2seq PLMs. DeSel improves greedy search by an average of 4.7% semantic F1 across five datasets. Our collective findings pave the way for deeper future investigations into PLM-based KPG.

==> figures/various_bert_models.tex <==
% \begin{figure}[h]
%     \centering
%     \small
%     \resizebox{\linewidth}{!}{
%     \begin{tabular}{ p{0.98\linewidth} }
%     \toprule
%     \textbf{Academic domain} \\
%     \hdashline \\
%     [-2ex]
%     SciBERT \citep{beltagy-etal-2019-scibert}, BioBERT \citep{Lee_2019}, ChemBERTa \citep{2010.09885}, [Bio|CS]\_RoBERTa \citep{gururangan-etal-2020-dont}, BioMegatron \citep{shin-etal-2020-biomegatron}, MatSciBERT \citep{2109.15290}, PubMedBERT \citep{Gu_2022}, MatBERT \citep{TREWARTHA2022100488}, BatteryBERT \citep{huang2022batterybert}  \\
%     \midrule \\ 
%     [-2ex]
%     \textbf{Social domain}  \\
%     \hdashline \\
%     [-2ex]
%     ClinicalBERT \citep{alsentzer-etal-2019-publicly}, FinBERT \citep{2006.08097}, LEGAL-BERT \citep{chalkidis-etal-2020-legal}, JobBERT \citep{zhang-etal-2022-skillspan}, PrivBERT \citep{srinath-etal-2021-privacy}, SportsBERT \citep{sportsbert} \\
%     % \footnote{\textcolor{red}{(https://huggingface.co/microsoft/SportsBERT)}} \\
%     \midrule \\ 
%     [-2ex] 
%     \textbf{Web domain}  \\
%     \hdashline \\
%     [-2ex]
%     Twitter-roberta \citep{barbieri-etal-2020-tweeteval}, BERTweet \citep{nguyen-etal-2020-bertweet},  [News|Reviews]\_RoBERTa \citep{gururangan-etal-2020-dont}, HateBERT \citep{caselli-etal-2021-hatebert} \\
%     \bottomrule
%     \end{tabular}}
%     \vspace{-2mm}
%     \caption{
%     Domain-specific encoder-only PLMs are available in a variety of domains. No prior work considered using these "domain experts" for keyphrase generation.
%     }
%     % \vspace{-2mm}
%     \label{various-bert-models}
%     % \vspace{-2mm}
% \end{figure}


\begin{figure}[h]
    \centering
    \small
    \resizebox{\linewidth}{!}{
    \begin{tabular}{ c | c | c  }
    \toprule
    \textbf{Model Name} & \textbf{Reference} &\textbf{Domain} \\ 
    \midrule
    SciBERT & \citet{beltagy-etal-2019-scibert} & Science \\
    BioBERT & \citet{Lee_2019} & Science \\
    ChemBERTa & \citet{2010.09885} & Science \\
    Bio\_RoBERTa & \citet{gururangan-etal-2020-dont} & Science \\
    CS\_RoBERTa & \citet{gururangan-etal-2020-dont} & Science \\
    BioMegatron & \citet{shin-etal-2020-biomegatron} & Science \\
    MatSciBERT & \citet{2109.15290} & Science \\
    PubMedBERT & \citet{Gu_2022} & Science \\
    MatBERT & \citet{TREWARTHA2022100488} & Science \\ 
    BatteryBERT & \citet{huang2022batterybert} & Science \\
    \hdashline
    ClinicalBERT & \citet{alsentzer-etal-2019-publicly} & Social \\
    FinBERT & \citet{2006.08097} & Social  \\
    LEGAL-BERT & \citet{chalkidis-etal-2020-legal} & Social  \\
    JobBERT & \citet{zhang-etal-2022-skillspan} & Social  \\
    PrivBERT & \citet{srinath-etal-2021-privacy} & Social  \\
    SportsBERT & \citet{sportsbert} & Social  \\
    \hdashline
    Twitter-roberta & \citet{barbieri-etal-2020-tweeteval} & Web \\
    BERTweet & \citet{nguyen-etal-2020-bertweet} & Web  \\
    News\_RoBERTa & \citet{gururangan-etal-2020-dont} & Web  \\
    NewsBERT & this work & Web \\
    Reviews\_RoBERTa & \citet{gururangan-etal-2020-dont} & Web  \\
    HateBERT & \citet{caselli-etal-2021-hatebert} & Web  \\
    \bottomrule
    \end{tabular}}
    \vspace{-2mm}
    \caption{
    Domain-specific encoder-only PLMs are available in a variety of domains. No prior work considered using these "domain experts" for keyphrase generation.
    }
    % \vspace{-2mm}
    \label{various-bert-models}
    % \vspace{-2mm}
\end{figure}


